Comparison of Autoscaling Frameworks for Containerised Machine-Learning-Applications in a Local and Cloud Environment

When deploying machine learning (ML) applications, the automated allocation of computing resources-commonly referred to as autoscaling-is crucial for maintaining a consistent inference time under fluctuating workloads. The objective is to maximize the Quality of Service metrics, emphasizing performance and availability, while minimizing resource costs. In this paper, we compare scalable deployment techniques across three levels of scaling: at the application level (TorchServe, RayServe) and the container level (K3s) in a local environment (production server), as well as at the container and machine levels in a cloud environment (Amazon Web Services Elastic Container Service and Elastic Kubernetes Service). The comparison is conducted through the study of mean and standard deviation of inference time in a multi-client scenario, along with upscaling response times. Based on this analysis, we propose a deployment strategy for both local and cloud-based environments.

==> RelatedWork.tex <==
\section{Related work}
Autoscaling has become a highly frequented research field. Most work focuses on the development of autoscaling rules. A common technique is the use of machine learning algorithms like reinforcement learning \cite{Khaleq}\cite{Hamid}\cite{Khaleq2}\cite{Joyce}, decision trees \cite{Abdullah}\cite{Vu} or long short term models \cite{Marie-Magdelaine}. Further methods are based on multi-level metric monitoring \cite{Taherizadeh}, fuzzy logic \cite{Tseng}, second order autoregressive moving average (ARMA) \cite{Roy} and simple moving average (SMA) \cite{Cheng}. Moreover, the combination of local predictors including support vector machines and ARMA \cite{Kim} or long short term memory neural networks and autoregressive integrated moving average \cite{Radhika} are used. While most autoscaling techniques focus on horizontal scaling, vertical scaling \cite{Jang} and combinations of both \cite{Kwan}\cite{Ding} are also of great interest. Reference \cite{Podolskiy} compare the autoscaling services of three cloud provider (Amazon Web Services, Microsoft Azure, Google Cloud Platform) on virtual machine (VM) and container level. To our best knowledge, there has been no research conducted to compare container and application level autoscaling in a ML-specific task in a local and cloud environment.
